VITA: Versatile Time Representation Learning for Temporal Hyper-Relational Knowledge Graphs

Knowledge graphs (KGs) have become an effective paradigm for managing real-world facts, which are not only complex but also dynamically evolve over time. The temporal validity of facts often serves as a strong clue in downstream link prediction tasks, which predicts a missing element in a fact. Traditional link prediction techniques on temporal KGs either consider a sequence of temporal snapshots of KGs with an ad-hoc defined time interval or expand a temporal fact over its validity period under a predefined time granularity; these approaches not only suffer from the sensitivity of the selection of time interval/granularity, but also face the computational challenges when handling facts with long (even infinite) validity. Although the recent hyper-relational KGs represent the temporal validity of a fact as qualifiers describing the fact, it is still suboptimal due to its ignorance of the infinite validity of some facts and the insufficient information encoded from the qualifiers about the temporal validity. Against this background, we propose VITA, a $\underline{V}$ersatile t$\underline{I}$me represen$\underline{TA}$tion learning method for temporal hyper-relational knowledge graphs. We first propose a versatile time representation that can flexibly accommodate all four types of temporal validity of facts (i.e., since, until, period, time-invariant), and then design VITA to effectively learn the time information in both aspects of time value and timespan to boost the link prediction performance. We conduct a thorough evaluation of VITA compared to a sizable collection of baselines on real-world KG datasets. Results show that VITA outperforms the best-performing baselines in various link prediction tasks (predicting missing entities, relations, time, and other numeric literals) by up to 75.3%. Ablation studies and a case study also support our key design choices.

==> backup.tex <==


% % This fact implies that Barack Obama has already completed his degree at Harvard University. Consequently, the relationship \textit{"Educated at"} should have a lower probability of being a valid potential relationship compared to others, as it refers to a past event. To address this limitation, temporal knowledge graphs (TKGs) are introduced, which incorporate temporal information into facts. In TKGs, each fact is extended with a timestamp or time period, resulting in a quadruple structure. For example, the quadruple \textit{{Barack Obama, Educated at, Harvard University, [1988, 1991]}} indicates that this fact is only valid from 1988 to 1991, as illustrated in Figure \ref{fig:IntroFact}b. However, there are two major challenges in link prediction for TKGs. First, TKG models struggle to capture the rich semantics of each fact because the quadruple structure does not account for the qualifiers introduced in HKGs. Second, TKG models often suffer from redundancy in representing facts with different types of time intervals. For instance, models like TeMP \cite{TeMP}, T-GAP \cite{T-GAP}, and TARGCN \cite{TARGCN} create a series of facts for each timestamp within a valid time interval or across the entire timeline, leading to excessive duplication.

% To address the aforementioned challenges, we propose the Temporal Hyper-relational Knowledge Graph (THKG), which integrates both HKG and TKG facts. THKG provides a universal representation of facts that can express rich semantics as well as temporal information. For example, a temporal hyper-relational fact \textit{{(Barack Obama, Educated at, Harvard University), (Occurperiod, 1988, 1991), (Academic degree, Juris Doctor), (Academic major, Law)}} can be divided into three distinct parts: the triplet representing the basic relationship, the temporal information representing the time interval (start and end times), and the qualifiers representing additional semantics. If the start or end time is missing, it is denoted by a -, signifying an infinite time period. Like traditional KGs, TKGs, and HKGs, THKGs are also incomplete, necessitating link prediction to infer missing facts. However, existing KG, HKG, and TKG LP models are not suitable for this new type of fact structure. Therefore, in this paper, we not only introduce new datasets formatted for THKGs, but also propose a novel model specifically designed for THKG LP.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{img/IntroFact.png}
%     \caption{A Comparison between HKG's fact, TKG's fact and THKG's fact.}
%     \label{fig:IntroFact}
% \end{figure}

% We propose four datasets: \todo{}. For the first two, we extend Wikidata11k \cite{T-GAP} and YAGO1830 \cite{xERTE} from temporal knowledge graph (TKG) datasets into \todo{} by collecting the qualifiers for each fact. Then, we extend wd50k \city{StarE} from hyper-relation knowledge graph (HKG) datasets into by collecting the temporal information for each fact. Finally, we scale and restructure wikipeople \cite{NaLP}, as these datasets already include temporal information in qualifiers, but it is incomplete. The key difference is that \todo{} contain both time-sensitive and time-invariant facts simultaneously.

% To learn the triplet, temporal information, and qualifiers respectively, we first designed \todo{}, which can capture the structural features of each module. This allows the contextual features of each part of the fact to be learned and aggregated using a transformer model. Additionally, we consider that some facts occur within specific time periods, meaning different facts should follow a chronological order. To achieve this, we further design a \todo{} to fuse chronological information using a cosine function. Finally, we design several \todo{} components to decode the temporally fused contextual features.
